Multimodal Trustworthy Semantic Communication for Audio-Visual Event Localization

The exponential growth in wireless data traffic, driven by the proliferation of mobile devices and smart applications, poses significant challenges for modern communication systems. Ensuring the secure and reliable transmission of multimodal semantic information is increasingly critical, particularly for tasks like Audio-Visual Event (AVE) localization. This letter introduces MMTrustSC, a novel framework designed to address these challenges by enhancing the security and reliability of multimodal communication. MMTrustSC incorporates advanced semantic encoding techniques to safeguard data integrity and privacy. It features a two-level coding scheme that combines error-correcting codes with conventional encoders to improve the accuracy and reliability of multimodal data transmission. Additionally, MMTrustSC employs hybrid encryption, integrating both asymmetric and symmetric encryption methods, to secure semantic information and ensure its confidentiality and integrity across potentially hostile networks. Simulation results validate MMTrustSC's effectiveness, demonstrating substantial improvements in data transmission accuracy and reliability for AVE localization tasks. This framework represents a significant advancement in managing intermodal information complementarity and mitigating physical noise, thus enhancing overall system performance.

==> 1_introduction.tex <==
\section{Introduction}




\noindent \textbf{Background}


\noindent \textbf{Motivations.}

\noindent \textbf{Challenges.}
\subsubsection{\textcolor{red}{Security Analysis}}
Cryptography algorithms ensure that the information transmitted over public channels remains confidential even if intercepted, thus safeguarding messages and data. For virtually all standard cryptographic algorithms, successful decryption hinges not only on possessing the correct decryption key but also on the ciphertext being intact.
However, in traditional channel semantic coding, where the conveyed information resides in the domain of real numbers, even minute errors can be tolerated as they do not prevent the accurate recovery of the relevant features of the semantic information. This discrepancy often results in the output from the decoder differing slightly from the original message, presenting a challenge to the encryption and protection of semantic information using standard cryptographic methods.
As discussed previously, we have devised a dual-layer coding system to achieve reliable channel encoding and decoding. By adding an outer layer of error-correcting code to conventional channel encoders, minor weight errors potentially introduced by the traditional encoder-decoder pair can be secondarily corrected, ensuring absolute fidelity of the output information.
With the aid of reliable channel encoders and decoders, we can ascertain that the information input into the encoder and the output from the decoder are identical, laying the groundwork for the transmission of ciphertext by the sender and its subsequent decryption by the receiver.
In this paper, we employ the concept of hybrid encryption to realize the secure transmission of semantic information. Specifically, we first establish a shared secure session key between the sender and the receiver using public-key cryptography principles. Subsequently, this session key is used to symmetrically encrypt the information to be transmitted.
This approach leverages the strengths of both public-key and symmetric-key cryptography, combining the ease of key distribution from the former with the efficiency and speed of the latter for data encryption. The result is a robust framework for secure communication capable of maintaining confidentiality and integrity across potentially hostile networks. 

\noindent \textbf{Contributions.}


























-------------------------------------------------------
\IEEEPARstart{I}{n} current communication systems, the exponential growth of wireless data traffic due to the increasing number of mobile devices and expanding smart demands presents new challenges. Traditional communication systems require data conversion into bits at the transmitter and accurate bit recovery at the receiver, demanding high channel conditions and signal-to-noise ratios. Semantic communication, in contrast, directly transmits and retrieves the meaning of transmitted content, making it more robust in complex channel conditions~\cite{qin2019deep,shi2021new}.

Addressing the challenges of multimodal semantic communication currently focuses mainly on single-modal tasks~\cite{xie2021task,xie2022task}. However, in multimodal tasks, enhancing inter-modal information complementarity and semantic enrichment are crucial. Physical noise during channel transmission exacerbates inter-modal information interference, thereby affecting the execution of multimodal tasks and diminishing system performance.

Furthermore, existing semantic communication relies on joint source-channel coding, which poses risks such as information leakage and insecurity in transmitting multimodal data. For instance, scenarios requiring concurrent processing of audio and video may struggle to maintain the integrity and privacy of multimodal data using traditional methods.

Regarding the integrity and privacy of multimodal data, further analysis reveals that in semantic communication, the encoding and decoding process involves semantic coding and channel coding. This process introduces two types of noise: semantic noise due to information loss during semantic encoding/decoding, and channel noise arising from physical channel disturbances. These noises contribute to semantic loss and interference among multimodal information, leading to unreliable multimodal information and hindering the implementation of multimodal tasks.

Moreover, multimodal information faces risks of external attacks and information leakage both at the sender and receiver ends. In semantic communication, leakage of information may occur due to insufficient encryption during transmission or inadequate protection of storage devices. Therefore, this article proposes enhancing semantic encryption of multimodal semantic information at the sender's semantic encoding stage to prevent information leakage and tampering. At the receiver's semantic decoding stage, decrypting semantics helps correct errors introduced during encoding/decoding processes, enhancing resilience against semantic and physical noise interference. This approach effectively improves the accuracy of multimodal information transmission and supports the execution of multimodal tasks.

In summary, by incorporating encryption protection and semantic error correction mechanisms into multimodal semantic communication, the system can effectively mitigate security risks and various noise interferences during transmission, thereby enhancing system robustness, reliability, and ensuring the integrity and privacy of multimodal data.

In this letter, we provide multimodal trustworthy semantic communication for multimodal semantic recognition task (Audio-Video Event Localization, AVE).
\begin{figure*}[!th]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/framework_new.png}
    % \vspace{-1.7cm}
    \caption{The framework of Multimodal Trustworthy Semantic Communication (MMTrustSC) for the Multimodal AVE Task.}
    \label{fig:framework}
\end{figure*}
\begin{itemize}
    % \item \textbf{Novel Framework.} We provide a famework of Multimodal Trustworthy Semantic Communication for Multimodal Task, referred to Multi\_TSC. 
    \item We introduce a novel framework, named TrustworthyMultiSem, specifically designed to ensure secure and reliable transmission of multimodal semantic information for AVE localization tasks. This framework integrates advanced semantic encoding techniques to safeguard data integrity and privacy throughout transmission.
    \item TrustworthyMultiSem utilizes state-of-the-art semantic encoding and decoding techniques to mitigate semantic noise and channel noise, ensuring robust transmission and accurate reception of multimodal data essential for AVE localization.

\item At the core of TrustworthyMultiSem is a comprehensive approach to semantic encryption at the transmitter, safeguarding multimodal semantic information from unauthorized access and manipulation during transmission. The receiver side employs semantic decryption mechanisms to effectively restore and utilize received data for precise AVE localization.

\item Practical simulations conducted demonstrate the effectiveness of TrustworthyMultiSem in maintaining the fidelity of transmitted multimodal semantic information, thereby facilitating accurate AVE localization through the seamless integration and processing of audio and visual data.
\end{itemize}
